Reversible Programming: A Case Study of Two String-Matching Algorithms

String matching is a fundamental problem in algorithm. This study examines the development and construction of two reversible string-matching algorithms: a naive string-matching algorithm and the Rabin-Karp algorithm. The algorithms are used to introduce reversible computing concepts, beginning from basic reversible programming techniques to more advanced considerations about the injectivization of the polynomial hash-update function employed by the Rabin-Karp algorithm. The results are two clean input-preserving reversible algorithms that require no additional space and have the same asymptotic time complexity as their classic irreversible originals. This study aims to contribute to the body of reversible algorithms and to the discipline of reversible programming.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{G.W. Hamilton, T. Kahsai, M. Proietti (Eds.):\\
Joint International Workshops on \\
Horn Clauses for Verification and Synthesis (HCVS 2022)\\
Verification and Program Transformation (VPT 2022)\\
EPTCS 373, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.373.1}{10.4204/EPTCS.373.1}}
\pdfoutput=1

